Reproducible Aggregation of Sample-Split Statistics

Statistical inference is often simplified by sample-splitting. This simplification comes at the cost of the introduction of randomness not native to the data. We propose a simple procedure for sequentially aggregating statistics constructed with multiple splits of the same sample. The user specifies a bound and a nominal error rate. If the procedure is implemented twice on the same data, the nominal error rate approximates the chance that the results differ by more than the bound. We illustrate the application of the procedure to several widely applied econometric methods.

==> old_text.tex <==
To fix ideas, consider the setting of \cite{banerjee2015multifaceted}, who study data collected from a randomized evaluation of a poverty alleviation program implemented in several developing countries.\footnote{Further details on our treatment of the \cite{banerjee2015multifaceted} data are given in \cref{app: simulation appendix}.} We focus on their evaluation of the effect of the program on the level of household consumption in Bangladesh. For each household in their sample, they observe a vector $D_i = (Y_i, W_i, X_i)$, where $Y_i$ is a measurement of consumption three years after the implementation of the program, $W_i$ is an indicator denoting assignment to the program, and $X_i$ is a vector of pretreatment covariates. Let $D= (D_i)_{i=1}^n$ collect the data in their sample. 

The augmented inverse propensity score weighted (AIPW) estimator of \cite{robins1994estimation} is a standard approach to estimating average treatment effects in randomized experiments. This estimator is formed by randomly splitting the sample into two parts. Let $\mathsf{s}$ and $\tilde{\mathsf{s}}$ denote sets containing the indices of the households in each part. Using data from the households $i$ in $\tilde{\mathsf{s}}$, nonparametric estimates of the propensity score and conditional outcome regression
\[
\pi(x) = P\{W_i = 1 \mid X_i = x\} \quad \text{and} \quad \mu_w(x) = \mathbb{E}[Y_i  \mid X_i = x, W_i = w] 
\]
are formed. For example, conditional outcome regressions are often estimated with the Lasso estimator of \cite{tibshirani1996regression}, through
\begin{equation}
\hat{\mu}_w(X_i) = \hat{\beta}_w(\lambda) ^\top X_i, 
\quad\text{where}\quad 
\hat{\beta}_w(\lambda) = \underset{\beta}{\arg\min} \left\{
\sum_{i\in\tilde{\mathsf{s}}} \mathbb{I}\{W_i = w\} (Y_i - \beta^\top X_i)^2 + \lambda \|\beta\|_1 \right\}\label{eq: intro lasso}
\end{equation}
for some penalization parameter $\lambda$, with $\mathbb{I}\{ \cdot \}$ denoting the indicator function.\footnote{For the purposes of this section, we choose the penalization parameter with a single implementation of $10$-fold cross-validation of the mean-squared error. Similarly, we estimate the propensity score with a linear probability model constructed with $10$-fold cross-validated lasso. Further details on design of our simulation are given in \cref{app: simulation appendix}.} Collect these estimates into $\hat{\eta}(D_{\tilde{\mathsf{s}}}) = (\hat{\pi},\hat{\mu}_w)$, where $D_{\tilde{\mathsf{s}}}$ collects the data with indices in $\tilde{\mathsf{s}}$. The AIPW estimator is given by
\begin{align}
\label{eq: dml ate}
T(\mathsf{s},D) &= \frac{1}{\vert\mathsf{s}\vert}\sum_{i \in \mathsf{s}} \psi(D_i, \hat{\eta}(D_{\tilde{\mathsf{s}}})),\quad\text{where} \\
\psi(D_i, \hat{\eta}(D_{\tilde{\mathsf{s}}})) & = \hat{\mu}_1(X_i) - \hat{\mu}_0(X_i)
+ \frac{W_i(Y_i - \hat{\mu}_1(X_i))}{\hat{\pi}(X_i)}
- \frac{(1 - W_i)(Y_i - \hat{\mu}_0(X_i))}{1 - \hat{\pi}(X_i)}.\nonumber
\end{align}
Let $\mathsf{s}$ and $\mathsf{s}^\prime$ denote independently drawn subsets of $[n]=\{1,\ldots,n\}$ of size $n/2$. Panel A of \cref{fig: ate} compares the densities of the single-split, double-split, and two-fold cross-split estimators
\begin{equation}
\label{eq: one split, two split}
T(\mathsf{s},D),
\quad
\frac{1}{2}(T(\mathsf{s},D)+ T(\mathsf{s}^\prime,D)),
\quad\text{and}\quad 
\frac{1}{2}(T(\mathsf{s},D)+ T(\tilde{\mathsf{s}},D)),
\end{equation}
over repeated samples of $(\mathsf{s},\mathsf{s}^\prime)$ for the \cite{banerjee2015multifaceted} data.

\begin{figure}[t]
\begin{centering}
\caption{Residual Randomness}
\label{fig: ate}
\medskip{}
\begin{tabular}{cc}
\textit{Panel A: One Split, Two Splits} & \textit{Panel B: $10$-Fold Cross Split}\tabularnewline
\includegraphics[scale=0.4]{../build/2_demonstration/single_split} & \includegraphics[scale=0.4]{../build/2_demonstration/cross_split_10}\tabularnewline
\multicolumn{2}{c}{\textit{Panel C: $10$-Fold Cross Validation}}\tabularnewline
\multicolumn{2}{c}{\includegraphics[scale=0.4]{../build/2_demonstration/lasso_intro}}\tabularnewline
\end{tabular}
\par\end{centering}
\medskip{}
\justifying
{\footnotesize{}Notes: Panel A of \cref{fig: ate} displays kernel estimates of the density of the single split, double split, and two-fold cross split estimators defined in \eqref{eq: one split, two split} over repeated samples of $(\mathsf{s},\mathsf{s}^\prime)$ for the \cite{banerjee2015multifaceted} data. Panel B displays a discretized heat map of the joint distribution of the 10-fold cross split estimator $a(\mathsf{r}_{10},D)$ defined in \eqref{eq: k fold dml} and the critical value estimator $\mathsf{CV}_{\alpha}(\mathsf{r}_{10},D)$ defined in \eqref{eq: k fold dml cv}. The black line denotes the threshold where the estimator is equal to the estimated critical value. Panel C displays quantiles of the $10$-fold cross-validated estimate of the mean-squared error \eqref{eq: risk estimate} of the Lasso regression \eqref{eq: intro lasso} over a grid of values of $\lambda$. The probabilities that each value of $\lambda$ minimizes the cross-validated risk estimate are displayed with large grey dots.}{\footnotesize\par}
\end{figure}

The variability in the estimator across sample-splits is substantial and sufficient to switch the sign. A moderate increase in the number of splits does not address the problem. The $k$-fold cross-split estimator is given by 
\begin{equation}
\label{eq: k fold dml}
a(\mathsf{r}_{k},D) = \frac{1}{k}\sum_{j=1}^k T(\mathsf{s}_j,D)~,
\end{equation}
where $\mathsf{r}_k = (\mathsf{s}_i)_{i=1}^k$ is a collection of $k$ equally sized sets that form a partition of $[n]$.\footnote{If $\pi$ and $\mu_w$ are estimated sufficiently well, this estimator is semiparametrically efficient for the average effect of the program on household consumption \citep{chernozhukov2018double,hahn1998role}.} An asymptotically exact test of the null hypothesis that the average effect of the program is less than or equal to zero can be constructed by comparing \eqref{eq: k fold dml} with the critical value
\begin{equation}
\label{eq: k fold dml cv}
\mathsf{CV}_{\alpha}(\mathsf{r}_k,D) = \frac{z_{1-\alpha}}{n} \left(\sum_{j=1}^k \sum_{i \in  \mathsf{s}_j} \left(\psi(Y_i, \hat{\eta}(D_{\tilde{\mathsf{s_j}}})) - a(\mathsf{r}_k,D) \right)^2 \right)^{1/2}~,
\end{equation}
where $z_{1-\alpha}$ is the $1-\alpha$ quantile of the standard normal distribution \citep{chernozhukov2018double}.  Panel B of \cref{fig: ate} displays a heat map of the joint distribution of the 10-fold cross-split statistic $a(\mathsf{r}_{10},D)$ and the critical value $\mathsf{CV}_{0.05}(\mathsf{r}_{10},D)$ over random draws of the partition $\mathsf{r}_{10}$. The residual variability in the estimator has been greatly reduced, but is still large relative to estimates of the sampling variability. The choice of the partition $\mathsf{r}_{10}$ determines whether a test that the treatment effect of the program is negative is rejected. 

The problem of residual variability is even more severe when choosing the penalization parameter $\lambda$ in the Lasso regression \eqref{eq: intro lasso} with cross-validation. Here, the sample-split statistic of interest is the out-of-sample mean-squared error estimate
\begin{equation}
\label{eq: risk estimate}
T(\mathsf{s}, D) = \frac{1}{\sum_{i\in\mathsf{s}}\mathbb{I}\{W_i = w\}} \sum_{i\in\mathsf{s}} \mathbb{I}\{W_i = w\} (Y_i - \hat{\beta}_w(\lambda)^\top X_i)^2~.
\end{equation}
Often, the penalization parameter $\lambda$ is chosen as the value that minimizes the cross-fit statistic \eqref{eq: k fold dml}. Panel C of \cref{fig: ate} displays the distribution of $10$-fold cross-validated estimates of the mean-squared error of the regression \eqref{eq: intro lasso}, with $w$ equal to one, over a grid of values of $\lambda$.\footnote{We consider the values of $\lambda$ reported by the ``glmnet'' R software package \citep{friedman2021package}.} The probabilities that each value of $\lambda$ minimizes the cross-validated risk estimate are displayed with large grey dots. There is substantial variability in the penalization parameter chosen by $10$-fold cross-validation.

The primary methodological contribution of this paper is the introduction of a computationally efficient procedure for aggregating sample-split statistics across multiple splits to ensure that residual variability is small. The proposal is based on the sequential fixed-width confidence intervals developed by \cite{anscombe1952large} and \cite{chow1965asymptotic}. In \cref{sec: Reproducible}, we detail the proposed algorithm and give very general conditions for its validity, in a particular asymptotic sense.

A user must make several choices when implementing the procedure. These include specifying a suitable bound and error rate as well as choosing the size and joint distribution of the random splits. The primary theoretical contribution of this paper is a non-asymptotic analysis that motivates approaches for making these choices. In particular, in \cref{sec: theoretical analysis}, we restrict attention to linearly separable statistics that are symmetric in each part of each split. We give two main results. First, we derive concentration inequalities for averages of independently drawn cross-split statistics of the form \eqref{eq: k fold dml} around their conditional mean. Our bounds characterize the dramatic difference between the residual variability of the double split and two-fold cross split statistics displayed in Panel A of \cref{fig: ate}. Second, we provide a Berry-Esseen type bound on the accuracy of the nominal error rate for the procedure. As the procedure is sequential, this calculation is nonstandard. This result illustrates a trade-off between the computational efficiency of the procedure and the accuracy of the nominal error rate.

The main theoretical challenge posed by this analysis is the accommodation of the dependence between statistics computed on cross-splits of a sample. That is, conditioned on the data, the summands, over $j$ from $1$ to $k$, of the aggregate statistic \eqref{eq: k fold dml} will be dependent. We address this through an application of the method of exchangeable pairs \citep[see e.g.,][]{stein1986approximate, ross2011fundamentals,chen2011normal}. To construct an appropriate exchangeable pair for our problem, we develop a novel application of a coupling argument due to \cite{chatterjee2005concentration}. See also \cite{paulin2013deriving,paulin2016efron}. The various concentration and moment inequalities we develop are then obtained by applying results due to \cite{chatterjee2005concentration,chatterjee2007stein}. These arguments are outlined in \cref{sec: proof outline}.

In \cref{sec: applications}, we measure the performance of our procedure in the applications considered in \cref{fig: ate}. \cref{sec: conclusion} concludes. Details concerning the data and simulations considered in this paper are given in \cref{app: simulation appendix}. Unless otherwise specified, proofs for all results stated in the main text are given in \cref{app: proof of main text}. Proofs supporting Lemmas used in \cref{app: proof of main text} are given in \cref{app: auxiliary}. \cref{app: additional} gives additional results that will be introduced at appropriate points throughout the paper.

\subsection{Related Literature} The procedure studied in this paper is based on the sequential fixed-width confidence intervals of \cite{anscombe1952large} and \cite{chow1965asymptotic}. Our non-asymptotic analysis is related to the Berry-Esseen bounds for randomly indexed sums given in \cite{landers1976exact, landers1988sharp}. Applications of these results to  fixed-width confidence intervals have been given in \cite{csenki1980convergence}, \cite{ mukhopadhyay1981convergence}, and \cite{callaert1981convergence}. A more recent non-asymptotic consideration of the application of fixed width confidence intervals to Monte Carlo techniques is given in \cite{hickernell2013guaranteed}. Our more specialized analysis differs from these results by accommodating and quantifying the dependence induced by cross-splitting. 

Our setting is related to a large literature that studies methods for constructing confidence intervals for cross-validated estimates of generalization error. Several recent examples include \cite{dietterich1998approximate}, \cite{nadeau1999inference}, \cite{lei2020cross}, \cite{bayle2020cross}, \cite{austern2020asymptotics}, and \cite{bates2023cross}. In contrast, we are interested in the randomness conditional on the data. Formally, our results are most similar to the Berry-Esseen bounds given in \cite{austern2020asymptotics}, who study the unconditional normal approximation of statistics similar to the those considered in \cref{sec: theoretical analysis}. Our bounds apply under strictly weaker conditions and are substantially simpler. See also \cite{chetverikov2021cross} and \cite{chetverikov2021analytic} for further analyses of cross-validated regression. 

Some of our arguments build on a literature studying the role of algorithmic stability in the accuracy of cross-validation \citep{kale2011cross,kumar2013near}. These papers are related to a broader literature that derives generalization bounds for stable algorithms, originating with \cite{bousquet2002stability}. The stability of several specific estimators is studied in \cite{elisseeff2005stability}, \cite{hardt2016train}, \cite{celisse2016stability}, \cite{chen2022debiased}, and \cite{du2023extrapolated}. Some of the concentration inequalities we derive can be compared to the results of \cite{cornec2010concentration} and \cite{abou2019exponential}. Again, the setting we study is different and our conditions are substantially simpler.

\cite{chen2022debiased} show that sample-splitting is unnecessary for the asymptotic normality of estimators of the form \eqref{eq: dml ate} if the nuisance parameter estimator $\hat{\eta}$ satisfies a stability condition related to some of the conditions studied in this paper. The intention of our paper is not to argue that sample-splitting should, necessarily, be used for any particular application. Rather, our premise is that sample-splitting is widely applied in practice, irrespective of its optimality.

The procedure studied in this paper is applicable to a large variety of statistical methods constructed with sample-splitting. General methods for testing statistical hypothesis with sample-splitting are studied in \cite{guo2017analysis}, \cite{romano2019multiple}, \cite{diciccio2020exact}, \cite{wasserman2020universal}, and \cite{tse2022note}. \cite{rinaldo2019bootstrapping} study a general procedure for selective inference based on sample-splitting. \cite{meinshausen2009p} and \cite{meinshausen2010stability} study methods for inference in high-dimensional linear models that use multiple data splitting. \cite{chernozhukov2018generic} study a procedure for estimating best linear predictors of heterogeneous treatment effects based on sample-splitting.

Although our emphasis is on statistics constructed with sample-splitting, the algorithmic and formal methods studied in this paper are potentially applicable to randomized algorithms more generally. See \cite{beran1987stochastic} for an analysis of the asymptotics of randomized tests and estimators. \cite{guo2023rank} and \cite{zhang2023framework} propose methods for conducting inference with randomized algorithms through subsampling \citep{politis1999subsampling}.

\subsection{Notation}
We let $\tilde{\mathsf{s}}$ denote the complement of the set $\mathsf{s}$ in $[n]=\{1,\ldots,n\}$. The set $\mathcal{S}_{n,b}$ consists of all subsets of $\left[n\right]$ of size $b$. The set $\mathcal{R}_{n,k,b}$ contains all collections of $k$ mutually exclusive elements of $\mathcal{S}_{n,b}$. We refer to elements of $\mathcal{R}_{n,k,b}$ as cross-splits. That is, if $n=k\cdot b$, then $\mathcal{R}_{n,k,b}$ is the set of all partitions of $[n]$ into $k$ mutually exclusive subsets of size $b$. Likewise, $\mathcal{R}_{n,1,b}$ is the collection of sets containing one element of $\mathcal{S}_{n,b}$. We say $a\lesssim b$ if there exists a universal constant $C$ such that $a\leq Cb$.  We let $z_\alpha$ denote the $\alpha$ quantile of the standard normal distribution and $\lfloor x\rfloor$ denote the largest integer smaller than or equal to $x$.

\section{Reproducible Aggregation \label{sec: Reproducible}}

Consider a sample $D = (D_i)_{i=1}^n$. Let $\mathsf{s}$ be some subset of $\left[n\right]$ with complement $\tilde{\mathsf{s}}$. We are interested in reporting a real-valued sample-split statistic of the form 
\begin{equation}
T\left(\mathsf{s}, D \right)=
\Psi \left(D_\mathsf{s}, \hat{\eta} \left(D_{\tilde{\mathsf{s}}}\right)\right),\label{eq: test statistic}
\end{equation}
where the collection $D_\mathsf{s}=(D_{i})_{i\in\mathsf{s}}$
contains data with indices in $\mathsf{s}$, $\hat{\eta}$ is an estimator of an unknown nuisance parameter $\eta$, and $\Psi\left(\cdot\right)$ is some function.
The structure encoded in statistics of the form \eqref{eq: test statistic} is quite general and encompasses most applications of sample-splitting encountered in practice, including out-of-sample evaluation of prediction error, model selection, and nuisance parameter estimation.

We study methods for aggregating statistics of the form \eqref{eq: test statistic} across multiple splits of the same sample. Our objective is to ensure that the auxiliary randomness introduced by sample-splitting is small. In particular, for each collection $\mathsf{R}_{g,k}=(\mathsf{r}_i)_{i=1}^g$ of $g$ elements of $\mathcal{R}_{n,k,b}$, where we write $\mathsf{r}_i = (\mathsf{s}_{i,j})_{j=1}^k$, we consider aggregate statistics of the form
\begin{equation}
a(\mathsf{R}_{g,k}, D)=\frac{1}{g}\frac{1}{k}\sum_{i=1}^{g}\sum_{j=1}^{k}T(\mathsf{s}_{i,j},D)~.\label{eq: aggregate}
\end{equation}
The statistic \eqref{eq: aggregate} generalizes several standard methods for aggregating sample-split statistics. If $k=n/b$ and $g=1$, then \eqref{eq: aggregate} is a $k$-fold cross-split statistic (also known as, e.g., $k$-fold cross-validation or $k$-fold cross-fitting). If $k=1$, then \eqref{eq: aggregate} averages over $g$ independently drawn sample-splits. In this case, if $\hat{\eta}$ is constant, then \eqref{eq: aggregate} is an incomplete $U$-statistic of order $b$.\footnote{A special case of the class of statistics with $k=1$ are subsampled statistics \citep{politis1999subsampling}.} We entertain the intermediate cases, i.e., where $k$ is between $1$ and $n/b$, so that the theoretical results to follow interpolate between independent splitting and cross-splitting. Throughout, we denote the proportion $b/n$ by $\varphi$.

Our task is to formulate a method for choosing the number of collections of mutually exclusive splits $g$ to ensure that the residual variability of the aggregate statistic \eqref{eq: aggregate} is small. This objective is formalized in the following criterion.
\begin{defn}[Reproducibility]  \label{def: reproducibility} Suppose that the integers $\hat{g}$ and $\hat{g}^\prime$ and the collections $\mathsf{R}_{\hat{g},k}$ and $\mathsf{R}^\prime_{\hat{g}^\prime,k}$,  are independent and identically distributed, conditional on the data $D$. We say that $\mathsf{R}_{\hat{g},k}$ is $(\xi,\beta)$-reproducible if
\begin{equation}
P\bigg\{\big\vert a(\mathsf{R}_{\hat{g},k}, D) - a(\mathsf{R}^\prime_{\hat{g}^\prime,k}, D) \big\vert \leq \xi \mid D\bigg\} \geq 1 - \beta \label{eq: Reproducibility}
\end{equation}
almost surely. 
\end{defn}

\begin{remark}
Suppose that the data $D$ are given to two researchers. Each researcher is tasked with producing an estimate of the form \eqref{eq: aggregate}. They generate the collections of splits $\mathsf{R}_{\hat{g},k}$ and $\mathsf{R}^\prime_{\hat{g}^\prime,k}$ independently using the same procedure. That is, the two collections of splits used by the two researchers are independent and identically distributed conditional on the data $D$. If this procedure is $(\xi,\beta)$-reproducible, then the probability that the two researchers' estimates differ by more than $\xi$ is less than $\beta$.\hfill$\blacksquare$
\end{remark}

We propose a sequential method for constructing a reproducible collection $\mathsf{R}_{\hat{g},k}$. Our proposal is based on the fixed-length sequential confidence intervals of \cite{anscombe1952large} and \cite{chow1965asymptotic}. Define the variance estimator
\begin{flalign}
\label{eq: var estimator}
\hat{v}\left(\mathsf{R}_{g,k}, D\right) & 
=\frac{1}{g\left(g-1\right)k^{2}}\sum_{i=1}^{g}\sum_{j,j^{\prime}=1}^{k}
\left(T(\mathsf{s}_{i,j},D)-a\left(\mathsf{R}_{g,k}, D\right)\right)
\left(T(\mathsf{s}_{i,j^{\prime}},D)-a\left(\mathsf{R}_{g,k}, D\right)\right).
\end{flalign}
Observe that \eqref{eq: var estimator} is simply the sample variance of the summands in \eqref{eq: aggregate} across the $g$ collections of splits. Our procedure iteratively draws a collection uniformly at random and computes the variance \eqref{eq: var estimator} until the condition 
\begin{equation}
\label{eq: empirical stopping time}
\hat{v}\left(\mathsf{R}_{g,k}, D\right) \leq \mathsf{cv}_{\xi,\beta} = \frac{1}{2}\left(\frac{\xi}{z_{1-\beta/2}}\right)^2
\end{equation}
is satisfied. We let $\hat{g}$ denote the smallest value of $g$ greater than or equal to $g_{\mathsf{init}}$ such that \eqref{eq: empirical stopping time} is satisfied, where $g_{\mathsf{init}}\geq2$ is an integer chosen by the user. This procedure is summarized in \cref{alg: sequential aggregation}.

\begin{algorithm}[t]
\caption{Anscombe-Chow-Robbins Aggregation} \label{alg: sequential aggregation}
\KwIn{Data $D$, tolerance $\xi$, error rate $\beta$, collection size $k$, split size $b$, initialization $g_{\mathsf{init}}$}

Set $g \leftarrow g_{\mathsf{init}}$

Draw $\mathsf{r}_1$, ..., $\mathsf{r}_{g_{\mathsf{init}}}$ independently and uniformly from $\mathcal{R}_{n,k,b}$.  Collect $\mathsf{R}_{g_{\mathsf{init}},k} = ( \mathsf{r}_j)_{j=1}^{g_{\mathsf{init}}}$.

\While{$\hat{v}(\mathsf{R}_{g,k}, D) > \mathsf{cv}_{\xi,\beta} $}{

Set $g \leftarrow g + 1$

Draw $\mathsf{r}_g$ uniformly from $\mathcal{R}_{n,k,b}$. Collect $\mathsf{R}_{g,k} = (\mathsf{R}_{g-1}, \mathsf{r}_g)$.

}
Set $\hat{g} \leftarrow g$

\Return $\mathsf{R}_{\hat{g},k}$

\end{algorithm}
\smallskip

The following theorem gives an asymptotic sense in which the collection of sample-splits chosen with \cref{alg: sequential aggregation} are $(\xi, \beta)$-reproducible. The proof is closely related to the arguments of \cite{anscombe1952large} and \cite{chow1965asymptotic}. See e.g., Theorem 3.1 of \citet{gut2009stopped} for a textbook treatment.
\begin{theorem}
\label{eq: general reproducibility}
Suppose that the real-valued statistic $a(\mathsf{R}_{1,k}, D)$ has a non-zero variance conditional on $D$ almost surely. If the collections $\mathsf{R}_{\hat{g},k}$ and $\mathsf{R}^\prime_{\hat{g}^\prime,k}$ are independently computed with \cref{alg: sequential aggregation}, then
\begin{equation}
\label{eq: almost sure reproduce}
P\bigg\{\big\vert a(\mathsf{R}_{\hat{g},k}, D) - a(\mathsf{R}^\prime_{\hat{g}^\prime,k}, D) \big\vert \leq \xi \mid D\bigg\} \to 1 -\beta
\quad
\text{as}\quad\xi\to0~.
\end{equation}
\end{theorem}

\begin{remark}
\cref{eq: general reproducibility} applies to a fixed data set $D$. Asymptotics are taken as $\xi \to 0$ with all other quantities, including the sample size $n$, fixed. Roughly, \cref{eq: general reproducibility} is established by showing that
\begin{equation}
\label{eq: g star def}
\hat{g}/g^\star \overset{\text{a.s}}{\to} 1
\quad
\text{as}\quad\xi\to0,
\quad
\text{where}
\quad
g^\star
 = \min \left\{g : \Var\left(a(\mathsf{R}_{g,k}, D)\mid D\right) \leq \mathsf{cv}_{\xi,\beta}\right\}~,
\end{equation}
and using the fact that a central limit theorem will hold for the sequence $a(\mathsf{R}_{g^\star,k}, D)$ as $\xi\to0$, conditional on the data. The discrepancy between $a(\mathsf{R}_{\hat{g},k}, D)$ and $a(\mathsf{R}_{g^\star,k}, D)$ can be handled with an appropriate maximal inequality, an idea due to \citet{renyi1957asymptotic}.\hfill$\blacksquare$
\end{remark}

\begin{remark}
The proof of \cref{eq: general reproducibility} uses only the fact that the $g$ collections $\mathsf{r}_i$ in $\mathsf{R}_{g,k}$ are drawn independently and identically. However, \cref{fig: ate} suggests that we should expect the statistic $a(\mathsf{R}_{g,k}, D)$ to concentrate as $k$ increases. Some insight into this phenomenon can be gained without any assumptions. In particular, let $\mathsf{s}$ and $\mathsf{s}^\prime$ each be uniformly distributed on $\mathcal{S}_{n,b}$ such that their intersection is empty with probability one. Define the conditional variance and covariance
\begin{equation}
\label{eq: variance components}
\phi_{n,b}(D) = \Var(T(\mathsf{s}, D) \mid D)
\quad\text{and}\quad
\gamma_{n,b}(D) = \Cov(T(\mathsf{s}, D), T(\mathsf{s}^\prime, D) \mid D)
\end{equation}
respectively. We can evaluate
\begin{equation}
\label{eq: conditional variance}
v_{g,k}(D) = \Var(a(\mathsf{R}_{g,k}, D) \mid D) = \frac{1}{g}\left(\frac{1}{k}\phi_{n,b}(D) + \frac{k-1}{k}\gamma_{n,b}(D)\right).
\end{equation}
Observe that $\gamma_{n,b}(D) \leq \phi_{n,b}(D)$ by the Cauchy-Schwarz inequality. Thus, for a fixed total number of cross-splits $g$ and split size $b$, the conditional variance $v_{g,k}(D)$ decreases as $k$ increases. That is, cross-splitting (i.e., setting $k>1$) always has a smaller conditional variance than independent splitting (i.e., setting $k=1$) for a fixed value of $g$. On the other hand, for a fixed number of total splits $m=gk$ and split size $b$, the conditional variance $v_{g,k}(D)$ is smaller for cross-splitting than for independent splitting if and only if the conditional covariance $\gamma_{n,b}(D)$ is negative.

In many standard applications, the conditional covariance $\gamma_{n,b}(D)$ is negative.\footnote{This will not always be the case. In \cref{app: examples}, we give examples where $\gamma_{n,b}(D)$ obtains both endpoints of the Cauchy-Schwarz bound $-\phi_{n,b}(D)\leq\gamma_{n,b}(D)\leq\phi_{n,b}(D)$.} Consider again the \cite{banerjee2015multifaceted} data. \cref{fig: covariance} compares the variance components
\begin{equation}
\label{eq: cov terms}
\frac{1}{k}\phi_{n,b}(D)\quad\text{and}\quad-\frac{k-1}{k}\gamma_{n,b}(D)
\end{equation}
under the restriction that $n=kb$ for both the treatment effect and risk estimation applications introduced in \cref{eq: introduction}. In both cases, the two terms \eqref{eq: cov terms} are nearly equal, i.e., the two terms in the variance \eqref{eq: conditional variance} nearly cancel each other out. In other words, cross-splitting is able to account for almost all of the residual variability introduced by independent splitting. By placing restrictions on the statistic \eqref{eq: test statistic}, the subsequent section provides a non-asymptotic account of the error in the approximation \eqref{eq: almost sure reproduce} that quantifies and compares the concentration in $a(\mathsf{R}_{g,k}, D)$ with both $g$ and $k$.\hfill$\blacksquare$
\end{remark}

\begin{figure}[t]
\begin{centering}
\caption{Covariance Across Cross-Splits}
\label{fig: covariance}
\medskip{}
\begin{tabular}{cc}
\textit{Panel A: Treatment Effect Estimation} & \textit{Panel B: Risk Estimation}\tabularnewline
\includegraphics[scale=0.4]{../build/2_demonstration/cov_cross} & \includegraphics[scale=0.4]{../build/2_demonstration/cov_lass}\tabularnewline
\end{tabular}
\par\end{centering}
\medskip{}
\justifying
{\footnotesize{}Notes: \cref{fig: covariance} displays measurements of the quantities \eqref{eq: cov terms} for the treatment effect and risk estimation applications to the \cite{banerjee2015multifaceted} data introduced in \cref{eq: introduction}. For the risk estimation application, we study the regression \eqref{eq: intro lasso} for the treated outcome, i.e., $w$ equal to one, for a fixed choice of $\lambda$. In each case, the parameters $k$ and $b$ are chosen to satisfy $n=kb$. The $x$-axes are displayed in a log-scale base 10. Further details on this figure are given in \cref{app: simulation appendix}.}{\footnotesize\par}
\end{figure}

\section{Non-asymptotic Theory\label{sec: theoretical analysis}}

\cref{eq: general reproducibility} is very general. However, interpretation of the asymptotic approximation with $\xi\to0$ is somewhat nebulous, or at least unfamiliar. What would be a reasonable value of $\xi$ to choose such that the approximation \eqref{eq: almost sure reproduce} is accurate? Or, how quickly should we expect the error in \eqref{eq: almost sure reproduce} to diminish as $\xi$ shrinks?

We give a non-asymptotic analysis of the quality of the nominal error rate $\beta$ in \cref{alg: sequential aggregation}. This is accomplished by placing restrictions on the statistics of interest \eqref{eq: test statistic}. We emphasize that \cref{eq: general reproducibility} should provide assurance that \cref{alg: sequential aggregation} can be applied widely. The more specialized analysis that follows is aimed at (i) articulating why cross-split statistics often exhibit significantly lower residual variability than independently split statistics and (ii) providing intuition for how the error in the approximation \eqref{eq: almost sure reproduce} depends on the choices of $k$ and $\xi$. Proofs for results stated in this section are deferred to \cref{sec: proof outline}. 

\subsection{Symmetry, Linearity, and Stability}

We impose two simplifying restrictions on the statistic of interest. First, we assume that the statistic is symmetric and deterministic in each part of the split sample.
\begin{assumption}[Symmetry and Determinism]
\label{assu: invariance}For all sets $\mathsf{s}\subseteq[n]$
and data $D$, the statistic $T\left(\mathsf{s},D\right)$ is deterministic and invariant
to permutations of the data with indices in $\mathsf{s}$ and of the data with indices in $\tilde{\mathsf{s}}$. 
\end{assumption}
\begin{remark}
The intention of \cref{assu: invariance} is to restrict the residual randomness under consideration to the randomness introduced by sample-splitting. \cref{assu: invariance} rules out procedures where the estimator $\hat{\eta}$ is random conditional on the data. This includes settings where, e.g., $\hat{\eta}$ is estimated with stochastic gradient descent, bagging or subsampling, or is itself constructed with data splitting. It does not, however, exclude cases where $\hat{\eta}$ is deterministic, e.g., when $\hat{\eta}$ is a coefficient vector determined by a regularized regression or in the applications to hypothesis testing considered by \cite{diciccio2020exact} or \cite{wasserman2020universal}.\footnote{In \cref{app: test}, we show that the hypothesis tests constructed with multiple splits of the same sample considered in e.g., \cite{diciccio2020exact},  \cite{meinshausen2009p}, \cite{chernozhukov2018generic}, and \cite{wasserman2020universal} continue to be valid when they are constructed sequentially with \cref{alg: sequential aggregation}. These results follow from an inequality due to \cite{ramdas2023randomized}.}\hfill$\blacksquare$
\end{remark}
Second, we assume that the statistic \eqref{eq: test statistic} is linearly separable in the first part of the split sample.
\begin{assumption}[Linearity]
\label{assu: linearity}For all sets $\mathsf{s}\subseteq[n]$
and data $D$, the statistic $T\left(\mathsf{s},D\right)$ can be written
\begin{equation}
\label{eq: linear sep}
T\left(\mathsf{s},D\right) 
= \Psi \left(D_\mathsf{s}, \hat{\eta} \left(D_{\tilde{\mathsf{s}}}\right)\right) 
= \frac{1}{\vert \mathsf{s}\vert} \sum_{i\in\mathsf{s}} \psi(D_i, \hat{\eta} \left(D_{\tilde{\mathsf{s}}}\right))
\end{equation}
for some function $\psi(\cdot,\cdot)$.
\end{assumption}

\begin{remark}
\cref{assu: linearity} is satisfied in the applications to treatment effect and risk estimation studied in \cref{eq: introduction} in addition to the applications to hypothesis testing considered in \cite{diciccio2020exact} and \cite{wasserman2020universal}. Extending our analysis to cases where \eqref{eq: test statistic} satisfies a component-wise Lipschitz or bounded differences condition is worth further consideration.\hfill$\blacksquare$
\end{remark}

Both the remaining assumptions, and the ensuing bounds, specified in this section are expressed in terms of two objects that measure the sensitivity of the statistics of interest \eqref{eq: test statistic} to perturbations of the data and of the splits, respectively. We refer to these objects as stabilities.  Let $D^\prime$ denote an independent and identical copy of the data $D$. For each $\mathsf{q}\subseteq [n]$, let $\tilde{D}^{(\mathsf{q})}$ be constructed by replacing $D_i$ with $D^\prime_i$ in $D$ for each $i$ in $\mathsf{q}$.
\begin{defn}[Sample Stability] \label{def: sample stability}
 Fix a set $\mathsf{s}\subseteq\mathcal{S}_{n,b}$. Let $I$ be an index drawn uniformly from $\mathsf{s}$. Let $\mathsf{q}$ be a randomly selected subset of $\tilde{\mathsf{s}}$ of cardinality $q$. We refer to the quantities
\begin{align*}
\sigma_{\mathsf{valid}}^{(r)}
& =\mathbb{E}\left[
\big\vert 
\psi(D_I, \hat{\eta} \left(D_{\tilde{\mathsf{s}}}\right))
-
\psi(D^\prime_I, \hat{\eta} \left(D_{\tilde{\mathsf{s}}}\right))
\big\vert^{r}\right]
\quad\text{and}\\
\sigma_{\mathsf{train}}^{(r,q)}
&=\mathbb{E}\left[
\big\vert
\psi(D_I, \hat{\eta} \left(D_{\tilde{\mathsf{s}}}\right))
-
\psi(D_I, \hat{\eta} (\tilde{D}^{(\mathsf{q})}_{\tilde{\mathsf{s}}}))
\big\vert^{r}\right]
\end{align*}
as the $r$th-order validation and $(r,q)$th-order training sample stabilities, respectively. Similarly, we refer to the quantity 
\begin{equation} \label{eq: sample stability}
\sigma^{(r)}_{\mathsf{max}} = \max\left\{\sigma_{\mathsf{valid}}^{(r)}, \sigma_{\mathsf{train}}^{(r,1)}\right\}
\end{equation}
as the $r$th-order full sample stability.
\end{defn}
\begin{defn}[Split Stability] \label{def: split stability}
We refer to the quantity
\[
\zeta^{(r)}=\mathbb{E}\left[\max_{\mathsf{s},\mathsf{s}^{\prime}\in\mathsf{S}_{n,b}}\left(T\left(\mathsf{s},D\right)-T\left(\mathsf{s}^{\prime},D\right)\right)^{r}\right].
\]
as the $r$th-order split stability.
\end{defn} 
\noindent

At several points in the analysis that follows, we focus attention on statistics whose training sample stabilities shrink at an appropriate rate as $n$ increases. 
\begin{defn}\label{def: split stability}
A statistic $T\left(\mathsf{s},D\right)$ that satisfies \cref{assu: linearity} is sample stable if 
\begin{equation} \label{eq: training bound}
\sigma_{\mathsf{train}}^{(r,q)} \lesssim \left(\frac{q}{n-b}\right)^r
\end{equation}
uniformly for all even values of the parameter $r$. 
\end{defn} 
\begin{remark}
The $(2,1)$th-order training sample stability $\sigma_{\mathsf{train}}^{(2,1)}$ is a widely studied object and is referred to as mean-square stability in the statistical learning literature \citep[see e.g.,][]{kale2011cross,kumar2013near}.\footnote{Connections between sample stability and generalization are studied in \cite{bousquet2002stability} and \cite{celisse2016stability}.} In \cref{app: M estimation}, we give simple sufficient conditions for the sample stability of statistics that satisfy \cref{assu: linearity} when $\hat{\eta}$ is an empirical risk minimizer of a potentially regularized strictly convex loss. The argument is closely related to a similar result given in \cite{austern2020asymptotics}. Analogous bounds have been obtained for many estimators that do not necessarily satisfy \cref{assu: invariance}, such as bagged or subsampled estimators \citep{chen2022debiased}, ensemble methods \citep{elisseeff2005stability}, and estimators computed with stochastic gradient descent \citep{hardt2016train}. It most settings, it is reasonable to expect that the validation sample stability $\sigma_{\mathsf{valid}}^{(r)}$ is bounded for small values of $r$. The split stability $\zeta^{(r)}$ is a less frequently studied object, and we will only require that it is finite for $r$ equal to 4 or 8, depending on the setting. This is a weak restriction that will hold, for example, if  $T\left(\mathsf{s},D\right)$ is bounded.\hfill$\blacksquare$
\end{remark}

\subsection{Concentration and Normal Approximation\label{sec: concentration and normal approx}}
We begin by studying the concentration of the aggregate statistic $a(\mathsf{R}_{g,k}, D)$ about its conditional mean
\begin{equation} \label{eq: a bar}
\bar{a}\left(D\right) = \mathbb{E}\left[a(\mathsf{R}_{g,k}, D) \mid D\right] = \mathbb{E}\left[T(\mathsf{s}_{i,j},D) \mid D\right]~.
\end{equation}
The nonstandard aspect of our analysis is that we account for the dependence in the summands in $a(\mathsf{R}_{g,k}, D)$ across cross-splits, i.e., the dependence induced by cross-fitting. This is accomplished by constructing a suitable exchangeable pair with a coupling argument due to \cite{chatterjee2005concentration} and applying a method for deriving concentration inequalities with exchangeable pairs, also due to \cite{chatterjee2005concentration,chatterjee2007stein}. Aspects of our argument are closely related to the analysis of \cite{paulin2013deriving, paulin2016efron}.
\begin{theorem}
\label{thm: cross split concentration}Suppose that \cref{assu: invariance,assu: linearity} hold, that the data $D$ are independently and identically distributed, and that the statistic $a(\mathsf{R}_{1,k}, D)$ has a non-zero variance conditional on $D$ almost surely. If the fourth-order split stability $\zeta^{(4)}$ is finite, then the concentration inequality
\begin{align}
\log P\left\{ a(\mathsf{R}_{g,k}, D) - \bar{a}\left(D\right)
\geq t\mid D\right\} 
& \leq
- \frac{g}{2^4(2 - \varphi k - \varphi)^2} \frac{\delta t^2}{\Gamma_{k,\varphi,b}}
\label{eq: cross-splitting concentration}
\end{align}
holds with probability greater than $1-\delta$ as $D$ varies, where 
\begin{align}
\Gamma_{k,\varphi,b} & = \left(\frac{1-k\varphi}{1-\varphi}\right)4\sigma^{(2)}_{\mathsf{max}} + \left(\frac{k\varphi - \varphi}{1-\varphi}\right)\sigma^{(2,b-1)}_{\mathsf{train}}
\label{eq: Gamma 1 def}
\end{align}
and $\varphi = b/n$.
\end{theorem}

\begin{remark}
In the inequality \eqref{eq: cross-splitting concentration}, a conditional probability that depends on the data $D$ is bounded by a term that depends on the fixed parameters $g$, $k$, $\varphi$, $\delta$, and $t$ in addition to the unconditional quantity $\Gamma_{k,\varphi,b}$. In other words, if $\mathcal{F}$ is the event that the inequality \eqref{eq: cross-splitting concentration} holds, then $P\{\mathcal{F}\} > 1-\delta$ unconditionally. This transference from a conditional quantity to an unconditional quantity is obtained by a Markov type bound at one point in the proof. In the sequel, we give many conditional bounds of a similar form. This strategy---bounding the conditional quantities of interest with unconditional quantities---is helpful because the resultant unconditional objects are more tractable and are widely studied.\hfill\qed
\end{remark}

\begin{remark}
The quantity $\Gamma_{k,\varphi,b}$ interpolates between $\sigma^{(2)}_{\mathsf{max}}$ and $\sigma^{(2,b-1)}_{\mathsf{train}}$ as $k$ varies between its bounds $1$ and $1/\varphi$.\footnote{The pre-factor $(2 - \varphi k - \varphi)$ also reduces by a factor of 2 as $k$ increases from $1$ to $1/\varphi$.} In the case of independent splitting, the rate of concentration for the statistic $a(\mathsf{R}_{g,k}, D)$ is driven by the full sample stability $\sigma^{(2)}_{\mathsf{max}}$. On the other hand, in the case of cross-splitting, concentration depends only on the training sample stability $\sigma^{(2,b-1)}_{\mathsf{train}}$. At the extreme, if $b$ is set equal to one and $k$ is set equal to $n$, known as leave-one-out or jackknife cross-fitting, $\Gamma_{k,\varphi,b}$ will equal zero and there will be no residual randomness (that is, the assumption that $a(\mathsf{R}_{1,k}, D)$ has a non-zero conditional variance is violated).

To provide a quantitative sense of this tradeoff, \cref{fig: stability} displays estimates of $\sigma^{(2)}_{\mathsf{valid}}$ and $\sigma^{(2,b-1)}_{\mathsf{train}}$ for the risk and treatment effect estimation applications to the \cite{banerjee2015multifaceted} data, where we have approximated the unknown data generating distribution with the empirical distribution of the data. The training stability is dramatically smaller than the validation stability and decreases rapidly as $b$ decreases.

\begin{figure}[t]
\begin{centering}
\caption{Sample Stability}
\label{fig: stability}
\medskip{}
\begin{tabular}{cc}
\textit{Panel A: Treatment Effect Estimation} & \textit{Panel B: Risk Estimation}\tabularnewline
\includegraphics[scale=0.4]{../build/2_demonstration/stability_cross} & \includegraphics[scale=0.4]{../build/2_demonstration/stability_lass}\tabularnewline
\end{tabular}
\par\end{centering}
\medskip{}
\justifying
{\footnotesize{}Notes: \cref{fig: stability} displays estimates of the validation and training sample stabilities, defined in \cref{def: sample stability}, for the treatment effect and risk estimation applications to the \cite{banerjee2015multifaceted} data introduced in \cref{eq: introduction}. For the risk estimation application, we study the regression \eqref{eq: intro lasso} for the treated outcome, i.e., $w$ equal to one, for a fixed choice of $\lambda$. We approximate the unknown true data generating distribution with the empirical distribution of the data. The $y$-axes are displayed in a log-scale base 10. Further details on this figure are given in \cref{app: simulation appendix}.}{\footnotesize\par}
\end{figure}

An interesting structure emerges under the assumption that $T\left(\mathsf{s},D\right)$ is sample stable. In particular, restricting attention to the case of cross-fitting $b=n/k$, and plugging \eqref{eq: training bound} into the bound \eqref{eq: cross-splitting concentration} yields
\[
\frac{\delta g t^2}{2^4(1 - \varphi)^2} \left(\frac{n-b}{b-1}\right)^2 \geq \frac{\delta}{2^4} g k^2 t^2
\]
In other words, in the case of cross-splitting, large deviation probabilities converge to zero with an exponential rate that is quadratic in $k$. By contrast, the exponential rate of concentration is always linear in $g$. That is, for a fixed total number of splits $m=gk$, the exponential rates of concentration for sample stable statistics aggregated with independent splitting and with cross-splitting are $m$ and $m\cdot k$, respectively.\hfill$\blacksquare$
\end{remark}

Next, we derive bounds for the centered conditional moments of $a\left(\mathsf{R}_{g,k}, D\right)$ through an argument closely related to the proof of \cref{thm: cross split concentration}. Bounds of this form are known as Burkholder-Davis-Gundy inequalities \citep{burkholder1973distribution}. By combining these bounds with a standard Berry-Esseen inequality \citep{shevtsova2011absolute}, we obtain a non-asymptotic central limit theorem as a corollary.
\begin{theorem}
\label{cor: Moment bound}Suppose that \cref{assu: invariance,assu: linearity} hold and that the data $D$ are independent and identically distributed. If $r=2^{c-1}$ for some positive integer $c$ and the $4r$th-order split stability $\zeta^{(4r)}$ is finite, then the inequality
\begin{align}
\label{eq: applied BDG}
\mathbb{E}\left[\left(a\left(\mathsf{R}_{g,k}, D\right)-\bar{a}\left(D\right)\right)^{2r}\right]
 & \leq 
(2r-1)^r \left(\frac{2^4(2-\varphi k - \varphi)^2}{g}\right)^r \Gamma_{k,\varphi,b}^{(r)}~,
\end{align}
holds, where
\begin{align}
 \Gamma_{k,\varphi,b}^{(r)}   &= 
 \left(\frac{1-k\varphi}{1-\varphi}\right) 
 2^{2r} \sigma_{\mathsf{max}}^{(2r,1)} 
 + \left(\frac{k\varphi - \varphi}{1-\varphi}\right) \sigma_{\mathsf{valid}}^{(2r,b-1)}
\end{align}
and $\varphi = b/n$.
\end{theorem}

\begin{remark}
By setting $r=1$, the inequality \eqref{eq: applied BDG} gives a variance bound. In this case, the right-hand side of the inequality \eqref{eq: applied BDG} is equal to negative one times the inverse of the right-hand side of the inequality \eqref{eq: cross-splitting concentration}. In this sense, the concentration inequality \eqref{eq: cross-splitting concentration} can be thought of as an exponential Efron-Stein inequality adapted to the dependence inherent in our problem \citep{boucheron2003concentration}.\footnote{\cite{abou2019exponential} give related exponential Efron-Stein inequality in a different setting.} For values of $r$ greater than 1, the unconditional quantity $\Gamma_{k,\varphi,b}^{(r)}$ again interpolates between the $2r$th order full sample stability $\sigma_{\mathsf{max}}^{(2r,1)}$ and the $(2r,b-1)$th order training sample stability $\sigma_{\mathsf{valid}}^{(2r,b-1)}$ as $k$ increases from $1$ to $1/\varphi$. For sample stable statistics under cross-fitting, the bound  \eqref{eq: applied BDG} can be re-written
\begin{equation}
\label{eq: applied moment bound r gtr 1}
\mathbb{E}\left[\left(a\left(\mathsf{R}_{g,k}, D\right)-\bar{a}\left(D\right)\right)^{2r}\right]
\lesssim
\left(\frac{1}{gk^{2}}\right)^r
\end{equation}
by omitting constants that depend only on $r$. The rate of convergence of central moments of cross-split sample stable statistics is much faster with $k$ than it is with $g$. \hfill\qed
\end{remark}

The Kolmogorov distance between two measures $P$ and $Q$ on the
real line is given by 
\begin{equation}
\label{eq: kol dist def}
d_{\text{K}}\left(P,Q\right)=\sup_{w\in\mathbb{R}}\left\{ \vert P\left\{ (-\infty,w]\right\} -Q\left\{ (-\infty,w]\right\} \vert\right\} .
\end{equation}
With a mild abuse of notation, we let $d_{\text{K}}\left(X,Y\right)$
denote the Kolmogorov distance between the probability measures of
the real-valued random variables $X$ and $Y$.
\begin{cor} \label{thm: normal approximation}
Let $W$ denote a standard normal random variable. Suppose that \cref{assu: invariance,assu: linearity} hold, that the data $D$ are independently and identically distributed, and that the statistic $a(\mathsf{R}_{1,k}, D)$ has a non-zero variance conditional on $D$ almost surely. If the eighth-order split stability $\zeta^{(8)}$ is finite, then for all $g$, the conditional Berry-Esseen inequality
\begin{flalign}
\label{eq: cross-splitting berry esseen}
d_{\text{K}}\left(\frac{a\left(\mathsf{R}_{g,k}, D\right)-\bar{a}\left(D\right)}{\sqrt{v_{g,k}\left(D\right)}},W\bigg \vert D\right) & 
\leq
\frac{2^6 3^2}{\delta}\frac{\left(2-\varphi k-\varphi \right)^{3}}{g^{1/2}} \left(\frac{(\Gamma_{k,\varphi,b}^{(2)})^{1/2}}{v_{1,k}(D)}\right)^{3/2}
\end{flalign}
is satisfied with probability greater than $1-\delta$ as $D$ varies.\footnote{To the best of our knowledge, the only Stein's method central limit theorem in the Kolmogorov distance, applicable to our setting, is given in \cite{zhang2022berry}, which generalizes the argument of \cite{shao2019berry}. In \cref{app: zheng comparion}, we show that this central limit theorem implies a bound that does not reduce as either $g$ or $k$ increase.} 
\end{cor}

\begin{remark}
Consider again the case of cross-splitting, where $k=n/b=1/\varphi$. By \cref{cor: Moment bound}, the Berry-Esseen bound \eqref{eq: cross-splitting berry esseen} is at least
\begin{equation}
\frac{(1-\varphi)^3}{g^{1/2}}\left(\frac{(\sigma^{(4,b-1)}_{\mathsf{train}})^{1/2}}{v_{1,k}(D)}\right)^{3/2}
\gtrsim
\frac{1}{g^{1/2}}
\left(\frac{(\sigma^{(4,b-1)}_{\mathsf{train}})^{1/2}}{\sigma^{(2,b-1)}_{\mathsf{train}}}\right)^{3/2}~.\label{eq: berry esseen lower}
\end{equation}
Suppose that the statistic is sample stable. As long as $\sigma^{(4,b-1)}_{\mathsf{train}}$ and $\sigma^{(2,b-1)}_{\mathsf{train}}$ are well-approximated by their upper bounds \eqref{eq: training bound}, the quantity \eqref{eq: berry esseen lower} is of order $g^{-1/2}$ and does not decrease as $k$ increases. 

This argument suggests that, despite the fast decay in the residual randomness demonstrated in \cref{cor: Moment bound}, the quality of a normal approximation to $a\left(\mathsf{R}_{g,k}, D\right)$ does not increase as $k$ increases. This is again born out in our running examples. \cref{fig: kolmogorov} displays the Kolmogorov distance between a standard normal random variable and the studentized distribution of the cross-fit statistic $a\left(\mathsf{R}_{1,k}, D\right)$ conditioned on $D$ over a range of values of $k$ for our two applications to the \cite{banerjee2015multifaceted} data. That is, \cref{fig: kolmogorov} plots the left-hand side of the inequality \eqref{eq: cross-splitting berry esseen}. In both cases, despite a substantial initial improvement, the quality of a normal approximation does not increase for large $k$. In fact, in the risk estimation application, the quality of a normal approximation decays for values of $k$ larger than 20. On the other hand, it is worth noting that a normal approximation in the treatment effect application is remarkably accurate for values of $k$ larger than 20.\hfill$\blacksquare$
\begin{figure}[t]
\begin{centering}
\caption{Quality of Normal Approximation}
\label{fig: kolmogorov}
\medskip{}
\begin{tabular}{cc}
\textit{Panel A: Treatment Effect Estimation} & \textit{Panel B: Risk Estimation}\tabularnewline
\includegraphics[scale=0.4]{../build/2_demonstration/ks_cross} & \includegraphics[scale=0.4]{../build/2_demonstration/ks_lass}\tabularnewline
\end{tabular}
\par\end{centering}
\medskip{}
\justifying
{\footnotesize{}Notes: \cref{fig: kolmogorov} displays measurements of the Kolmogorov distance \eqref{eq: kol dist def} between a standard normal random variable and the studentized distribution of the cross-fit statistic $a\left(\mathsf{R}_{1,k}, D\right)$ conditioned on $D$ over a range of values of $k$ for our two applications to the \cite{banerjee2015multifaceted} data. This quantity is defined in the left hand side of the inequality \eqref{eq: cross-splitting berry esseen}. The $y$-axis of Panel A is displayed in a log-scale base 10. For the risk estimation application, we study the regression \eqref{eq: intro lasso} for the treated outcome, i.e., $w$ equal to one, for a fixed choice of $\lambda$. Further details on this figure are given in \cref{app: simulation appendix}.}{\footnotesize\par}
\end{figure}
\end{remark}

\subsection{Reproducibility\label{sec: nonasymp reproduce}}
We now return our attention to the sequential procedure for aggregating sample-split statistics formulated in \cref{sec: Reproducible}. Our main result is a Berry-Esseen type bound on the accuracy of the nominal error rate $\beta$ for the Anscombe-Chow-Robbins method specified in \cref{alg: sequential aggregation}. 
\begin{theorem}
\label{thm: stable symmetric reproduce}
Suppose that the statistic $a(\mathsf{R}_{1,k}, D)$ has a non-zero and variance, conditional on $D$, almost surely and that the collections $\mathsf{R}_{\hat{g},k}$ and $\mathsf{R}^\prime_{\hat{g}^\prime,k}$ are independently computed with \cref{alg: sequential aggregation}. If \cref{assu: invariance,assu: linearity} hold, the data $D$ are independent and identically distributed, and the eighth-order split stability $\zeta^{(8)}$ is finite, then the Berry-Esseen inequality
\begin{align}
 \bigg\vert P\bigg\{\big\vert a(\mathsf{R}_{\hat{g},k}, D) - a(\mathsf{R}^\prime_{\hat{g}^\prime,k}, D) \big\vert \leq \xi \mid D\bigg\} 
 - (1 - \beta) \bigg\vert 
&\lesssim \rho_{k,\varphi,b}(\xi,\beta \mid D) + \lambda_{k,\varphi,b}(\xi,\beta \mid D)~,\label{eq: reproduce BE bound}
\end{align}
holds with probability greater than $1-\delta$ as $D$ varies, for
\begin{align}
\rho_{k,\varphi,b}(\xi,\beta \mid D)  &=
\frac{\xi}{z_{1-\beta/2}} \frac{(2 - \varphi k - \varphi)^3 (\Gamma^{(2)}_{k,\varphi,b})^{3/4}}{\delta \left(v_{1,k}\left(D\right)\right)^{2}}\quad\text{and}\label{eq: rho term}\\
\lambda_{k,\varphi,b}(\xi,\beta \mid D)  &= \left(
\frac{\xi}{z_{1-\beta/2}}
\frac{(2-\varphi k-\varphi)^{4}\Gamma^{(1)}_{k,\varphi,b} (\Gamma_{k,\varphi,b}^{(2)})^{1/2}}{\delta^{3/2}(v_{1,k}\left(D\right))^{5/2}}
\right)^{1/2}~,\label{eq: lambda term}
\end{align}
where a multiplicative factor that grows logarithmically as $\xi$ shrinks has been omitted in writing \eqref{eq: lambda term} and an additional additive term that shrinks exponentially as $\xi$ shrinks has been omitted in writing \eqref{eq: reproduce BE bound}.
\end{theorem}

\begin{remark}
Recall the definition of the oracle stopping time $g^\star$ given in \eqref{eq: g star def}. The bound \eqref{eq: reproduce BE bound} is obtained by decomposing the approximation error into two terms. The first term involves the error in a normal approximation to the difference $a(\mathsf{R}_{g^\star,k}, D) - a(\mathsf{R}^\prime_{g^\star,k}, D)$ and contributes the term $\rho_{\varphi,k}(\xi,\beta \mid D)$. As $g^\star$ is deterministic conditional on $D$, a bound on this term follows from an argument very similar to the proof of \cref{thm: normal approximation}. The second term involves the differences $a(\mathsf{R}_{\hat{g},k}, D) - a(\mathsf{R}_{g^\star,k}, D)$ and $a(\mathsf{R}^\prime_{\hat{g}^\prime,k}, D) - a(\mathsf{R}^\prime_{g^\star,k}, D)$ and contributes the quantity $\lambda_{\varphi,k}(\xi,\beta \mid D)$. The key step in bounding these quantities involves deriving a high probability bound for the difference $\hat{g} - g^\star$. This follows by combining a concentration inequality analogous to \cref{thm: cross split concentration} for the conditional variance estimator $\hat{v}_{g,k}(D)$ with a Bernstein-type maximal inequality, due to \cite{steiger1970bernstein}.\hfill$\blacksquare$
\end{remark}

\begin{remark}
The dependence of the bound \eqref{eq: reproduce BE bound} on $\xi$ is sharp, at least up to the logarithmic factor. This follows from the examples given in \cite{landers1976exact, landers1988sharp}. Berry-Esseen type bounds on the coverage error of Anscombe-Chow-Robbins fixed-width sequential confidence intervals have been given in \cite{csenki1980convergence}, \cite{ mukhopadhyay1981convergence}, and \cite{callaert1981convergence}. Our result differs in several respects. Most importantly for our application, the dependence of our bound on the quantities $k$, $\varphi$, and $v_{1,k}(D)$ is explicit. We explore the structure of the bound through these terms in the following remark. Secondarily, we give an explicit characterization of the logarithmic factors in the bound by using Bernstein-type concentration inequalities, e.g., the bound given in \cref{thm: cross split concentration}, rather than moment bounds.\hfill$\blacksquare$
\end{remark}

\begin{remark}
Restrict attention again to the case of cross-fitting and assume that the statistic of interest is sample stable. We will refer to the procedure that uses the oracle stopping time $g^\star$ in the place of $\hat{g}$ as the oracle procedure. 
Observe that the oracle stopping time $g^\star$ is the unique integer that satisfies
\begin{equation}\label{eq: g star re def}
g^\star-1\leq2v_{1,k}(D)\left(\frac{z_{1-\beta/2}}{\xi}\right)^2 \leq g^\star~.
\end{equation}
Replacing the variance $v_{1,k}(D)$ by the bound derived in \cref{cor: Moment bound}, we get that $g^\star$ is proportional to
\begin{equation}\label{eq: g star}
\frac{2}{k^2}\left(\frac{z_{1-\beta/2}}{\xi}\right)^2~.
\end{equation}
Thus, if $m^\star = k g^\star$ is the total number of splits used by the oracle procedure, then $m^\star$ is proportional to $k^{-1}$ as $k$ increases with all other quantities held fixed. In other words, the total number of splits used by the oracle procedure decreases rapidly as $k$ increases. In the proof of \cref{thm: stable symmetric reproduce}, we give high probability bounds for $\vert g^\star - \hat{g}\vert$. Consequently, similar intuition will hold for \cref{alg: sequential aggregation}. That is, with high probability, the computational cost scales like $k^{-1}$ as $k$ increases.

On the other hand, by \cref{cor: Moment bound}, the leading term $\lambda_{k,\varphi,b}(\xi,\beta \mid D)$ in the bound \eqref{eq: reproduce BE bound} is at least
\begin{equation} \label{eq: be reproduce plug in cross}
\left(
\frac{\xi}{z_{1-\beta/2}}
\frac{1}{\delta^{3/2}(1-\varphi)}
\frac{(\sigma_{\mathsf{train}}^{(4,b-1)})^{1/2}}{(\sigma_{\mathsf{train}}^{(2,b-1)})^{3/2}}
\right)^{1/2}~.
\end{equation}
If $\sigma_{\mathsf{train}}^{(4,b-1)}$ and $\sigma_{\mathsf{train}}^{(2,b-1)}$ are proportional to their upper bounds \eqref{eq: training bound}, then the quantity \eqref{eq: be reproduce plug in cross} is of order
\begin{equation} \label{eq: accuracy approx}
\left(
\frac{\xi}{z_{1-\beta/2}}
\frac{k}{\delta^{3/2}}
\right)^{1/2}~,
\end{equation}
which is in turn of order $(g^\star)^{-1/4}$ by \eqref{eq: g star}. 

Comparison of the quantities \eqref{eq: g star re def} and \eqref{eq: accuracy approx} illustrates a fundamental trade-off in the performance of \cref{alg: sequential aggregation} over the choice of $k$. Increased values of $k$ reduce the conditional variance $v_{g,k}(D)$, and thereby, reduce the oracle sample size $g^\star$, easing computational cost. But as a consequence, the quality of the accuracy of the nominal error rate may deteriorate. In particular, at smaller values of $g$, the accuracy of the estimator $\hat{v}_{g,k}(D)$ for the conditional variance $v_{g,k}(D)$ will be lower, increasing the risk that $\hat{g}$ is smaller than  $g^\star$. The increased risk of early stopping decreases the probability that a result is reproducible. It is desirable, then, to choose values for $k$ and $\xi$ such that the variance $v_{1,k}(D)$ is small enough to make \cref{alg: sequential aggregation} computationally efficient, but not so small that the effective sample size $g^\star$ is too small for the nominal error rate $\beta$ to be accurate. \hfill\qed
\end{remark}

\section{Performance\label{sec: applications}}

We now study the performance of \cref{alg: sequential aggregation} in the applications to the \cite{banerjee2015multifaceted} data introduced in \cref{eq: introduction}. \cref{fig: performance} displays measurements of reproducibility error
\begin{equation}
P\bigg\{\big\vert a(\mathsf{R}_{\hat{g},k}, D) - a(\mathsf{R}^\prime_{\hat{g}^\prime,k}, D) \big\vert \geq \xi \mid D\bigg\} \label{eq: reproducibility error}
\end{equation}
when $\mathsf{R}_{\hat{g},k}$ and $\mathsf{R}^\prime_{\hat{g}^\prime,k}$ are obtained independently with \cref{alg: sequential aggregation} for the risk estimation application. \cref{fig: performance ate}, given in \cref{app: additional discussion}, displays analogous measurements for the treatment effect estimation application. We set the nominal error rate to $\beta=0.1$ and vary the values of $k$ and $\xi$.
\begin{figure}[p]
\begin{centering}
\caption{Reproducibility Error in Risk Estimation}
\label{fig: performance}
\medskip{}
\begin{tabular}{c}
\textit{Panel A: Early Stopping with $g_\mathsf{init}=2$}\tabularnewline
\includegraphics[scale=0.4]{../build/2_demonstration/lasso_coverage_2}\tabularnewline
\textit{Panel B: Reproducibility with $g_\mathsf{init}=10$}\tabularnewline
\includegraphics[scale=0.4]{../build/2_demonstration/lasso_coverage_10}\tabularnewline
\end{tabular}
\par\end{centering}
\medskip{}
\justifying
{\footnotesize{}Notes: \cref{fig: performance} displays measurements of reproducibility error \eqref{eq: reproducibility error} for \cref{alg: sequential aggregation} in the risk estimation application to the \cite{banerjee2015multifaceted} data. A dashed horizontal line is displayed at the nominal error rate $\beta=0.1$. The $x$-axes vary the bound $\xi$ and are displayed in a log-scale base 10. We study the regression \eqref{eq: intro lasso} for the treated outcome, i.e., $w$ equal to one, for a fixed choice of $\lambda$. To ease computation, we only display reproducibility error estimates for a $(\xi,k)$ pair if $g^\star$ is less than $10^4$. Further details on this figure are given in \cref{app: simulation appendix}.}{\footnotesize\par}
\end{figure}

Panel A displays measurements of the reproducibility error with the initialization $g_{\mathsf{init}}$ set equal to 2, the minimal feasible value. A transition is evident. For large values of $\xi$, the reproducibility error is monotonically decreasing in $k$. As $\xi$ decreases, this pattern reverses and the reproducibility probability approaches the nominal error rate. This phenomenon is caused by severe early stopping at large values of $\xi$. In particular, at large values of $\xi$, there is a substantial probability that $\hat{g}$ is chosen to be a very small value, e.g., 2 or 3, often several orders of magnitude less than $g^\star$.\footnote{In the risk estimation application, with $k=10$, $g^\star$ is 54.4 when $\xi$ is 10.4 and is 570.5 when $\xi$ is 3.2.} We document this behavior in \cref{fig: sample size}, given in \cref{app: additional discussion}.

This issue can be addressed through a very small increase in $g_{\mathsf{init}}$. Panel B displays measurements of the reproducibility error with the initialization $g_{\mathsf{init}}$ increased to 10. The nominal error rate is now substantially more accurate over the full support of values for $\xi$ considered. The moderate inaccuracy at larger values of $\xi$ has two sources. First, there is still some risk of early stopping at values of $g$ not much greater than $10$. Second, if $\xi$ is large relative to the conditional variance $v_{1,k}(D)$, ensuring that $\hat{g}$ is at least 10 can cause the reproducibility error to be close to 0. At moderate values of $\xi$, the trade off documented in \cref{sec: theoretical analysis} is apparent. As $k$ increases, the effective sample size $g^\star$ decreases, reducing the accuracy of the nominal error rate. \cref{fig: sample size}, given in \cref{app: additional discussion}, demonstrates that this inaccuracy can be largely explained by the error in the approximation of $g^\star$ with $\hat{g}$. For small values of $\xi$, at the level of precision likely to be of practical interest, the nominal error rate is very accurate. 


\section{Reccomendations for Proctice\label{sec: conclusion}}

We propose a method for sequentially aggregating randomized statistics to ensure that residual randomness is small. The method is applicable under very general conditions. By restricting the set of statistics under consideration, we give a non-asymptotic analysis of the performance of the method. We have two main findings. First, aggregation of sample-split statistics with cross-splitting reduces residual randomness at a much faster rate than for independent splitting. Second, cross-splitting does not necessarily improve the quality of the nominal error rate of the procedure. Thus, users navigate a tradeoff. Finer cross-splitting reduces the conditional variance of the aggregate statistic, reducing the computation needed to achieve a given bound on the residual randomness. But as a consequence, the quality of the nominal error rate may have also been reduced, limiting the user's ability to give a high quality estimate of the probability that their results are reproducible.

Our computational analysis has highlighted the substantial practical importance of choosing the initialization parameter $g_{\mathsf{init}}$ to be sufficiently large. By contrast, our theoretical analysis is agnostic to this issue. In the context of fixed-length sequential confidence intervals, \cite{mukhopadhyay1996sequential} study the choice of $g_{\mathsf{init}}$. They show that if $g_{\mathsf{init}}$ is chosen appropriately, a non-uniform asymptotic approximation to the coverage error, based on Edgeworth expansions due to \cite{aras1993asymptotic}, has a leading term of order $O(\xi^{2})$. This is a substantial improvement on the $O(\xi^{1/2})$ rate given in \cref{thm: stable symmetric reproduce}. Further research should give a non-asymptotic treatment of the choice of the parameter $g_{\mathsf{init}}$, aimed at assessing whether the $O(\xi^{1/2})$ rate can be improved through further assumptions and a principled choice of $g_{\mathsf{init}}$.
